Understanding Hackers' Work: An Empirical Study of Offensive Security Practitioners

Offensive security-tests are a common way to pro-actively discover potential vulnerabilities. They are performed by specialists, often called penetration-testers or white-hat hackers. The chronic lack of available white-hat hackers prevents sufficient security test coverage of software. Research into automation tries to alleviate this problem by improving the efficiency of security testing. To achieve this, researchers and tool builders need a solid understanding of how hackers work, their assumptions, and pain points. In this paper, we present a first data-driven exploratory qualitative study of twelve security professionals, their work and problems occurring therein. We perform a thematic analysis to gain insights into the execution of security assignments, hackers' thought processes and encountered challenges. This analysis allows us to conclude with recommendations for researchers and tool builders to increase the efficiency of their automation and identify novel areas for research.

==> high_level_org.tex <==
   \subsection{High-Level Project Organization}

    %\todo{This is a section, together with figure 1, that we could remove if space is needed, we might be missing the obvious ``report writing is tedious'' section though}
    
    \begin{figure}[!t]
    \centering
    \includegraphics[width=3.5in]{organisatorical}
    \caption{Generic Project Phases during a Security Assessment.}
    \label{high_level}
    \end{figure}
    
    While a hacker's heart lies in execution, \textbf{project management} rules need to be obliged. When questioned, the interviewees responded with the steps shown in Figure~\ref{high_level}. During \textit{pre-sales}, the type and duration of the project are discussed with the customer. A common theme was that customers lack knowledge of the different pen test options and choose inefficient ones. After accepting the project, a \textit{kick-off meeting} is performed to clarify expectations and the scope of offensive activities. After this, practitioners \textit{execute} the security assignment and \textit{report} findings. These steps are often performed in an agile manner: frequent rounds of status updates and customer feedback occur. \textit{Reports} detail how findings can be reproduced and suggest remediation steps. After the latter have been applied by the customer, an optional \textit{retest} can be performed as a means of regression testing. Report writing was commonly identified as a tedious task.
    
    Interviewees emphasized the \textbf{importance of social interactions} during security assignments. The commonly stated goal was to improve the client's security posture; creating a situation in which the client's personnel perceives the ongoing penetration test as hostile, reduces the chance of this goal being reached.
    
    When vulnerabilities are located in vendor- rather than in client-code, \textbf{public disclosure} is another potential venue of publication. Multiple interviewees had performed responsible disclosures but were very aware of the legal and economic risks that disgruntled or stonewalling vendors could impose. Two negative outcomes were observed: on the one hand, interviewees abstained from publicly disclosing bugs, leading to higher vendor patch latency and thus prolonging the longevity of potential 0-days; on the other hand, two interviewees stated that after negative disclosure experiences, they only perform full disclosure where results are immediately published without contacting the vendor first.
 
